Beyond Domain Gap: Exploiting Subjectivity in Sketch-Based Person Retrieval

Person re-identification (re-ID) requires densely distributed cameras. In practice, the person of interest may not be captured by cameras and, therefore, needs to be retrieved using subjective information (e.g., sketches from witnesses). Previous research defines this case using the sketch as sketch re-identification (Sketch re-ID) and focuses on eliminating the domain gap. Actually, subjectivity is another significant challenge. We model and investigate it by posing a new dataset with multi-witness descriptions. It features two aspects. 1) Large-scale. It contains over 4,763 sketches and 32,668 photos, making it the largest Sketch re-ID dataset. 2) Multi-perspective and multi-style. Our dataset offers multiple sketches for each identity. Witnesses' subjective cognition provides multiple perspectives on the same individual, while different artists' drawing styles provide variation in sketch styles. We further have two novel designs to alleviate the challenge of subjectivity. 1) Fusing subjectivity. We propose a non-local (NL) fusion module that gathers sketches from different witnesses for the same identity. 2) Introducing objectivity. An AttrAlign module utilizes attributes as an implicit mask to align cross-domain features. To push forward the advance of Sketch re-ID, we set three benchmarks (large-scale, multi-style, cross-style). Extensive experiments demonstrate our leading performance in these benchmarks. Dataset and Codes are publicly available at: https://github.com/Lin-Kayla/subjectivity-sketch-reid

==> figure/teaser.tex <==
\newlength{\teaserh}
\setlength{\teaserh}{0.15\linewidth}

\makeatletter\def\@captype{figure}\makeatother
\begin{minipage}{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{rebuttal/motivation_v3.pdf}
\end{minipage}
\begin{minipage}{.46\linewidth}
\captionof{figure}{{\torevise{A comparison of our Market-Sketch-1K dataset with existing sketch datasets\protect\footnotemark. The square and circle markers denote the object- and human-centric attributes respectively. Their diameter represents the subjectivity. Our dataset is featured in large-scale, subjective, multi-style, and semi-professional.}}}
\label{fig:intro_summary}
\end{minipage}

\footnotetext{\scriptsize VIPSL~\cite{gao2012face}, Memory-Aware~\cite{ouyang2016forgetmenot}, PKU-Sketch~\cite{pang2018cross}, QMUL-Shoe/Chair~\cite{yu2016sketch}, and Handbag~\cite{song2017deep}.}
% \makeatletter\def\@captype{table}\makeatother
% \begin{minipage}{.49\textwidth}
% \centering

% % \includegraphics[width=.72\linewidth]{introSummary_v9.pdf}\\
% % \hspace{-6mm}
% \setlength{\fboxrule}{2pt}
% \setlength{\fboxsep}{1pt}
% \fbox{
% \begin{tabular}
% {   @{\hspace{0mm}}c@{\hspace{1mm}} 
%     @{\hspace{0mm}}c@{\hspace{1mm}}
%     @{\hspace{0mm}}c@{\hspace{1mm}} 
%     @{\hspace{0mm}}c@{\hspace{0mm}}
% }
% % \arrayrulecolor{blue}\hline
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_A.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_C.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_D.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_F.pdf}\\\arrayrulecolor{blue!20}\hdashline
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_A.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_C.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_D.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_F.pdf}\\
% % \arrayrulecolor{blue}\hline
% \end{tabular}
% }
% % \resizebox{0.9\linewidth}{!}{
% % \begin{tabular}{y{100}|z{31}z{31}z{31}z{31}}
% %     {} & \multicolumn{2}{c}{\textbf{Face}} & \multicolumn{2}{c}{\textbf{Person}}\\
% %     {attributes} & \cite{gao2012face}
% %       & \cite{ouyang2016forgetmenot}
% %       & \cite{pang2018cross} 
% %       & Ours\\%\midrule
% %       \shline
% %     \# identities          & 200    & 100     & 200 & {996}\\
% %     %Artist (\#)           & --     & --      & 5   & 6 \\
% %     \# styles or types           & 5      & 4       & 1   & {6} \\
% %     \# camera views          & --     & --      & 2   & {6} \\
% %     \# total photos         & 200    & 10,030  & 400 & {32,668} \\
% %     \# total sketches       & 1000   & 400     & 200 & {4,763} \\
% %     avg. \# sketches/style   & 200    & 100 &   200 & 793.8 \\
% %     avg. \# sketches/ID      & 5      & 4       & 1   & 4.78 \\\hline
% %     zoom-in style factor         & \xmark & \xmark  & \xmark & \cmark\\
% % \end{tabular}}
% \end{minipage}
% \begin{minipage}{.48\linewidth}
% \captionof{figure}{\wz{A comparison of our Market-Sketch-1K dataset with existing datasets, including VIPSL~\cite{gao2012face}, Memory-Aware Forensic Sketch~\cite{ouyang2016forgetmenot}, PKU-Sketch~\cite{pang2018cross}, QMUL-Shoe/Chair~\cite{yu2016sketch}, and Handbag~\cite{song2017deep}. Our dataset is featured in large-scale, subjective, multi-style, and semi-professional.}}
% \label{fig:intro_summary}
% \end{minipage}
% \begin{tabular}{l}
%     \includegraphics[width=.72\linewidth]{introSummary_v9.pdf}\\
% \end{tabular}
% \hspace{-6mm}
% \setlength{\fboxrule}{2pt}
% \setlength{\fboxsep}{1pt}
% \fbox{
% \begin{tabular}
% {   @{\hspace{0mm}}c@{\hspace{1mm}} 
%     @{\hspace{0mm}}c@{\hspace{1mm}}
%     @{\hspace{0mm}}c@{\hspace{1mm}} 
%     @{\hspace{0mm}}c@{\hspace{0mm}}
% }
% % \arrayrulecolor{blue}\hline
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_A.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_C.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_D.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0011_F.pdf}\\\arrayrulecolor{blue!20}\hdashline
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_A.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_C.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_D.pdf}&
%     \includegraphics[height=\teaserh]{MarketSketchSamples/0021_F.pdf}\\
% % \arrayrulecolor{blue}\hline
% \end{tabular}
% }
% \captionof{figure}{Characteristics of our proposed Market-Sketch-1K dataset (b), comparing with the PKU-Sketch~\cite{pang2018cross} dataset (a). Data points with different shapes, colors, and filling patterns are used to represent images with different identities, sketch styles/camera views, and modalities, respectively. By arranging the same person images (denoted by the same shapes) in the same row, we show the difference between our dataset and the PKU-Sketch. \wzremove{Aside from a larger scale, our dataset zoom-ins the sketch style factor resulting from different artists' subjective cognition and painting styles, which has not been investigated by PKU-Sketch. [Best viewed in color]}\TODO{Change the figure, highlight our characteristics (not only the style), 1) semi-professional, 2) multi-style, 3), then put it here,}}


% \TODO{Change the figure, highlight our characteristics (not only the style), 1) semi-professional, 2) multi-style, 3), then put it here,}

%To facilitate the understanding, we use different shapes, colors, shades, and filling patterns to denote different persons, artists (sketch styles), camera views, and modalities, respectively. Shapes are arranged according to person identities, where each row shows samples of one identity. In addition to a larger scale, our dataset zoom-ins the problem of different sketch styles resulting from different artists, which has not been investigated by PKU-Sketch. In this paper, the sketch style attributes to an artist's subjective cognition and his painting style. [Best viewed in color]

%\wzx{ Samples with same identity are arranged in a same row, while samples with different identities are arranged in different rows. We can observe that style factor is entangled with the person identities factor in PKU-Sketch dataset. It is hard to explore the sketch style (resulting from different artists) using the PKU-Sketch dataset. each person is drawn by more than one sketch artist.}  \wzx{Best viewed in color.}

%\vspace{8mm}

==> section/5_diss.tex <==
% \section{Discussion}
% \label{sec:dis}

% \subsection{Discussion on settings}
% \TODO{Multi modality search}

% sketch vs attribute ....


% Other applications of this dataset

% \subsection{Discussion on our network}

% \TODO{
% \heading{The "Why don't you just use X? " question
% }}



% \subsection{Discussion on Market-Sketch-1K}
% \torevise{
% \heading{Balance/imbalance settings.} Since the artist $S_2$ and $S_4$ drew fewer sketches (\cf \tabref{exp_datasplit}), different identities have different numbers of sketches. To this end, we designed different settings in each benchmark, including balanced and imbalanced. The imbalance issue always occurs in real applications. We leave room for future works to address this issue. \figref{intro_ttmat} also shows that performances of different groups vary a lot. Some groups are more suitable for testing, while some groups are more suitable for training. It also requires us to design different settings for each benchmark. 
% }

% \TODO{other usages}
% sketch random erasure, generalization

% \heading{Necessity.} We can observe that, in benchmark II, our model trained using our dataset mostly performs well on PKU-Sketch. Especially, the result of total$\rightarrow$PX setting can even beat all state-of-the-art methods trained on PKU-Sketch. It is because models trained on PKU-Sketch may suffer from biases due to the limited quantity and uniform style. Besides, the evaluation protocol is also not reliable since PKU-Sketch only employs 50 identities for testing. So our Market-Sketch-1K dataset, featured in large-scale and multi-style, is necessary for the Sketch re-ID community.

% \paragraph{Application scenario.} \TODO{add this, maybe find in previous rebuttal, to give some examples. NOTE our current method is potential to incorporate with attribute or language }

\paragraph{Limitations and practicality.} Compared with photos, sketches lose identity discrimination information (\eg appearance color). Retrieving a person using a sketch is not as effective as using a photo. On the other hand, sketches are drawn by humans and based on witnesses' memory. A gap between the identity's natural appearance and an artist's understanding always exists. Once a photo of the target can be obtained, general re-ID technologies are preferred. However, the Sketch re-ID is practical because a photo query is not always available. Meanwhile, the system is less biased by the appearance color and is robust to cloth changing. Market-Sketch-1K facilitates the person retrieval in this practical application scenario and works as an essential supplement to the general re-ID datasets. 


\paragraph{Broader impact.} We should clarify that there is no privacy issue raised by Market-Sketch-1K. On the one hand, the re-ID problem may suffer from the privacy issue, which is mainly raised by the access control of data collection. Our dataset is built on a public dataset Market-1501 and just for research purposes, which does not have this kind of issue. On the other hand, we collected sketches drawn by 6 student artists and obtained their permission to use sketches for academic purposes.

% \TODO{include the permission}


% \TODO{future work...}
